Fano threefolds in positive characteristic II

Let $X$ be a smooth Fano threefold over an algebraically closed field of positive characteristic. Assume that $|-K_X|$ is very ample and each of the index and the Picard number is equal to one. We prove that $3 \leq g \leq 12$ and $g \neq 11$ for the genus $g$ of $X$. Moreover, we show that there exists no smooth curve on $X$ along which the blowup is Fano.

==> section-reply.tex <==
\section*{Reply to the referee}


Thank you very much for your many constructive suggestions. 
%and for reading the manuscript carefully. 
Below, I have included my replies to the referee. 
Following that, I have also included a copy of the revised version, with the changes highlighted in  {\cred red}. 


% I appreciate the valuable comments that have improved the article. 
% Below is our response to the comments by the referee B.

%except for very minor ones. 



% \section*{ToDo}

% \textcolor{green}{TODO of TANAKA: 
% \begin{enumerate}
% %\item D: (10). 
% %\item Editor reply: 2, F-vs-$F$. 
% %\item Page 8 check. 
% %\item French Abstract. Fourier, CTX. 
% \item Colour check. 
% \item Erase Sections?: Reply to... (Table of contents). 
% \end{enumerate}
% }




%\newpage





\vspace{5mm}



%\begin{center}
%{\large Reply to the referee B}
%\end{center}
\vspace{5mm}


%I appreciate the referee's valuable comments that have improved the article. I have followed all the referee's suggestions. In particular, I have added several paragraphs to the Introduction to make it more accessible. I have also fixed the typos. Below is our response to the referee's comments.


\begin{enumerate}\setlength{\itemsep}{0.3cm}
\item  
I directly followed your suggestion. 
\item
I directly followed your suggestion. 
\item
I directly followed your suggestion. 
\item
I directly followed your suggestion. 
\item 
Yes. Thank you for pointing it out. I have removed it. 
\item 
Thank you for pointing it out. I have added the definition of $\psi : Y \to Z$. 
\item
I directly followed your suggestion. 
\item 
%SKIPPED (page 38) 
%{\cred HORYU, although I added Subsection 2.2}
In this paper, $T_PX$ denotes the naively defined embedded tangent space in $\P^N_k$. 
%For an affine space $P \in \mathbb A^N_k \subset \P^N_k$, $T_PX \cap \mathbb A^N_k$ is the naively defined tangent space. %It is defined as the 
In order to clarify this point, I added (14) in Subsection 2.1. 
%(14) in Subsection 2.1. 
By definition, $T_PX$ is a linear subvariety of $\P^N_k$. 
If $X$ is a linear subvariety of $\P^N_k$, then $T_PL=L$. 
In particular, $T_P(T_PX) = T_PX$ whenever $X$ is a closed subscheme of  $\P^N_k$ and $P \in X$.  
\item
I directly followed your suggestion. 
\item
I directly followed your suggestion. 
\item 
Yes. It is a typo. Thanks for pointing it out. 
$Z$ should be $\wt{Z}$. 
As the former argument was ambiguous, I have added some details. 
First, I make $\wt{A}$ more explicit, i.e., I first define $\wt{A}$ and after that, $A$ is defined. 
Second, I added the following displayed equation 
\[
\wt{C} = (\wt{B})^{\wedge} =  (\wt{A}_{\m_{\wt{A}}})^{\wedge} 
= \widehat{\MO}_{\wt{Z}, P}
\]
to emphasise $\wt{C} = \widehat{\MO}_{\wt{Z}, P}$. 
\item
I directly followed your suggestion. 
\end{enumerate}


\medskip

Apart from the points pointed out by the referee, 
I have corrected the following two parts except for very minor changes. 


\begin{enumerate}
\item[(A)] Proof of Theorem 6.3. Proof of Step 1. 
I missed $17$, so I have corrected the proof. 
\item[(B)] I have added Lemma 10.7, in order to fix the proof of  
Proposition 10.8. Lemma 10.7 is also helpful to clarify the proof of Lemma 10.9. 
\end{enumerate}
\newpage


\setcounter{page}{1}



